A Structured Method for Compilation of QAOA Circuits in Quantum Computing

Quantum Approximation Optimization Algorithm (QAOA) is a highly advocated variational algorithm for solving the combinatorial optimization problem. One critical feature in the quantum circuit of QAOA algorithm is that it consists of two-qubit operators that commute. The flexibility in reordering the two-qubit gates allows compiler optimizations to generate circuits with better depths, gate count, and fidelity. However, it also imposes significant challenges due to additional freedom exposed in the compilation. Prior studies lack the following: (1) Performance guarantee, (2) Scalability, and (3) Awareness of regularity in scalable hardware. We propose a structured method that ensures linear depth for any compiled QAOA circuit on multi-dimensional quantum architectures. We also demonstrate how our method runs on Google Sycamore and IBM Non-linear architectures in a scalable manner and in linear time. Overall, we can compile a circuit with up to 1024 qubits in 10 seconds with a 3.8X speedup in depth, 17% reduction in gate count, and 18X improvement for circuit ESP.

==> Proof.tex <==
\section{Proof for Input Clique Graph on Linear Architecture} 
\label{sec:proof}
Given an n vertex clique graph that needs to be mapped onto a n qubit Linear Nearest Neighbor (LNN) architecture, we want to prove that the corresponding circuit for the graph can be executed in at most 2n-2 cycles O(n). Before proving that the pattern executes all gates between every qubit, we need to explain the pattern mathematically and provide an intuitive understanding of the cycles involved with the pattern.

\subsection{Intuition and Representation}

\subsubsection{Mathematical Representation of Pattern}

Let $Q_i$, i from ${0,1, … n-1}$, represent the $i^{th}$ qubit in the architecture. Let $P_i$, i from ${0,1, … n-1}$, represent the physical position in the architecture. In both cases, n is the number of qubits in the architecture. Thus, the location of $Q_i$ switches after a swap, but $P_i$ always remains constant.

Note the pattern repeats itself every 4 cycles:

Let $i$ $\in$ $\{$all even integers $\leq n - 2\}$. Then for all $i$

\begin{enumerate}
    \item Execute all gates on $P_{i}$-$P_{1+i}$ 
    \item Execute all gates on $P_{1+i}$-$P_{2+i}$
\item Swap all qubits on $P_{1+i}$-$P_{2+i}$
\item Swap all qubits on $P_{i}$-$P_{1+i}$
\end{enumerate}


This can be represented in loop format as shown in Fig.\ \ref{fig:pattern_loop}.\\

\iffalse
\begin{algorithm}
\caption{Clique n (even) mapping on LNN}
\begin{algorithmic}[1] 
\STATE T = 0

\WHILE{ T $< N/2$} 
\FOR{$i=0 ; i \leq N-2, i+= 2$}
    \STATE $CPHASE(P_i, P_{i+1})$
\ENDFOR
\FOR{$i=1 ; i \leq N-3; i+= 2$}
    \STATE $CPHASE(P_i, P_{i+1})$
\ENDFOR
\FOR{$i=1 ; i \leq N-3; i+= 2$}
    \STATE $SWAP(P_i, P_{i+1})$
\ENDFOR
\FOR{$i=0 ; i \leq N-2, i+= 2$}
    \STATE $SWAP(P_i, P_{i+1})$
\ENDFOR
\STATE $T += 1$
\ENDWHILE

\end{algorithmic}
\end{algorithm}
\fi

\subsubsection{Representation as 2 opposite direction streams}
Notice that one iteration of two consecutive SWAP cycles in CTAG sends any gate on an even position i, "up" 2 locations and any gate on an odd position i, "down" 2 locations (up means going in descending order with regards to i, down meaning ascending). It is shown in Fig.\ \ref{fig:cyclic}. The only exception to this rule are the qubits on the edge of the architecture, i.e when i = 0 and when i = n-2 or n-1. In these cases, the qubits in positions $P_0$ and $P_{n-1}$ switch direction. Thus, we can intuitively understand the pattern as 2 opposite direction streams "shaking hands" with each other (shaking hands being a metaphor for gate execution) as shown in Fig.\ \ref{fig:cyclic}.
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.30\textwidth]{figures/cycle_rep_v2.pdf}
    \caption{CTAG SWAP Effect: (a) The original two SWAP cycles, (b) and (c) Cyclic representation of the effect of the SWAPs}
    \label{fig:cyclic}
\end{figure}

It is also important to note the distinction between the patterns when N is odd versus when N is even. In both cases, when i$=$0, the qubit on $P_0$ goes to $P_1$. The difference appears on the other end. When N is odd, qubit on $P_{N-2}$ goes to $P_{N-1}$ and qubit on $P_{N-1}$ goes to $P_{N-3}$. When N is even, qubit on $P_{N-3}$ goes to $P_{N-1}$ while qubit on $P_{N-1}$ goes to $P_{N-2}$. 

\subsubsection{Derive Cycle in Pattern}
Notice that a cycle for the qubit location update  exists in the pattern. If we select an arbitrary qubit in the pattern, let's say $C_0$, we can define an ordering in the pattern based around $C_0$ as shown in Fig.\ \ref{fig:initial_mapping}. Essentially, after one outer loop iteration, $C_0$ will occupy the physical location $C_1$ was in and $C_1$ will occupy $C_2$'s position and so on. For example, Fig.\ \ref{fig:initial_mapping} shows the position of the qubits after 1 outer loop iteration in the algorithm for N=8.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.30\textwidth]{figures/distance_cycle_v2.pdf}
    \caption{Sample Cycle for n=8 after 1 outer loops}
    \label{fig:initial_mapping}
\end{figure}

The critical observation here is that in this example (N=8), any qubit $C_0$ in P1 will interact with qubits $C_7$ ($P_0$) and $C_6$ ($P_2$). More abstractly, we can say that $C_0$ in $P_1$ will always interact with $C_{N-1}$ and $C_{N-2}$. The similar applies to all other $P_i$, which means that a qubit in position $i$ will always act with the qubits of a certain relative distance away from it in the cycle representation of as shown in Fig.\ \ref{fig:initial_mapping}. Thus, formally, we can show that any qubit that follows a path $P_X$ to $P_Y$ in the pattern will interact with all other qubits in the cycle, $\{C_1, C_2, ... C_{N-1}\}$. 


\subsection{Proof}
We want to show all qubits interact with all other qubits in the cycle exactly once. We know the pattern executes in 2N-2 cycles, and executes the outer loop N/2 times. Notice that each qubit only interacts with N-1 neighbors and visits N/2 locations P. We can show that for any N/2 subset of positions P that an arbitrary qubit Q travels in the cycle, that Q will interact with all other N-1 qubits $C_{i}$ in the cycle.

\iffalse
\fixit{For any $C_i$ if it is at location $P_j$, $C_{i+1}$ will be at $P_{(i+1) mod N}$. Discuss cases for j = 1, $C_i$ interacts with $C_{(i-1) mod N}$ and $C_{(i-2) mod N}$} The distance between i and $(i-1) mod N$ is 1. ... Talk about the distance all the way to N-1. 
\fi

First we have to distinguish whether the arbitrary qubit in position $P_i$ is chosen from the upward stream (i is even) or the downward stream (i is odd).

If a qubit is chosen from the downward stream, we will notice that if the qubit $C_i$ is chosen from $P_1$, it will always interact with $C_{(i+N-1) mod N}$ and $C_{(i+N-2) mod N}$, $P_3$ with $C_{(i+N-3) mod N}$ and $C_{(i+N-4) mod N}$ ... until $P_{N-1}$ (if N is even) or $P_{N-2}$ (if N is odd), in which $P_{N-1}$ will interact with $C_{i+1}$ or $P_{N-2}$ will interact with $C_{i+1}$ and $C_{i+2}$. Thus, for any qubit located on $P_j$, where j is odd, it will interact with qubits $C_{(i+N-j) mod N}$ and $C_{(i+N-j-1) mod N}$.

If a qubit is chosen from the upward stream, we will notice the same pattern we did in the downward stream, but in reverse. The qubit $C_i$ chosen on $P_0$ will always interact with $C_{(i+1) mod N}$, $P_2$ with $C_{(i+2) mod N}$ and $C_{(i+3) mod N}$ ... until $P_{N-2}$ (if N is even) or $P_{N-1}$ (if N is odd), in which $P_{N-2}$ will interact with $C_{(i+N-1) mod N}$ and $C_{(i+N-2) mod N}$ or $P_{N-1}$ will interact with $C_{(i+N-1) mod N}$. Thus, for any qubit located on $P_j$, where j is even, it will interact with qubits $C_{(i+j) mod N}$ and $C_{(i+j+1) mod N}$.

Thus, if we have a qubit's path in the cycle from $P_X$ to $P_Y$, then we can derive the list of neighbor qubits it interacted with on its path. 

In the case where we pick $C_0$ starting at $P_1$, the case is trivial, as we simply visit all neighbors from $C_{N-1}$ to $C_{1}$ in descending order. The same applies if we select $P_{N-2}$ (if N is even) or $P_{N-1}$ (if N is odd) to be $C_0$. Then we visit all neighbors from $C_{1}$ to $C_{N-1}$ in ascending order. A slightly more complicated case is if we pick a qubit that has to switch streams sometime during its path. If we pick a Qubit $C_i$ starting at $P_j$, where j is even, then it will execute with neighbors $C_{(i+j+2T)(mod N)}$ and $C_{(i+j+2T+1)(mod N)}$ at time T. We are guaranteed to execute with all other qubits starting with T = 0, $C_{i+j+2(0) (mod N)}$ = $C_{i+j (mod N)}$ until T = (N/2)-1, $C_{i+j+2((N/2)-1)+1(mod N)} = C_{i+j+N-1(mod N)} = C_{i+j-1 (mod N)}$. Let k = i+j. Thus, we have the ordering of $\{C_{k (mod N)}, C_{k+1 (mod N)} ... C_{N-1}, C_{1}, ...  C_{k-1 (mod N)}\}$ . The same logic applies for if we pick a Qubit starting at $P_j$, where j is odd. Then it will execute with $C_{(N-(i+j+2T))(mod N)}$ and $C_{(N-(i+j+2T+1))(mod N)}$ which produces the ordering $\{C_{N-k(mod N)}, C_{N-k-1(mod N)} ... C_{1}, C_{N-1}, ... C_{N-k+1(mod N)}\}$.


\subsection{Discussion of the Odd Qubit Number Case}
There are slight differences in the $CTAG$ pattern when N is odd and when N is even. When the pattern has an odd number of qubits, instead of N/2 outer loops, it runs (N+1)/2 loops instead. In addition, instead of 2 swaps and 2 execution cycles, there is only 1 swap and 1 execution cycle in the last outer loop of the pattern. This does not change the fact that a cycle still exists within the pattern and only changes the end condition of the loop. 

==> methodology.tex <==
\subsection{Methodology}
\label{sec:basismethod}
In this section, we introduce the $CTAG$-$I$ algorithm to find an optimal initial mapping that minimizes circuit depth. This algorithm is only for circuits that can be reduced through initial mapping and not dynamic use of the pattern. We then propose a second algorithm, $CTAG$-$H$ which can be used for more general graphs and architectures by adopting a more heuristic approach than $CTAG$-$I$.

\subsubsection{CTAG-I For Input Graphs that Can be Optimized by Initial Mapping}

~~ \\
\noindent{\textbf{The A* Approach}} The A* approach we propose takes advantage of the fact that we can immediately identify the cycle in which a CPHASE gate executes between 2 qubits. Essentially, when we map a new logical qubit $q_i$ to a physical location $p_j$, we can find the last cycle that $q_i$ will execute among all other currently mapped qubits by using the pattern. We can use this fact to help guide our heuristic cost function in our A star framework.

The first step of our algorithm is to sort the vertices in the input problem graph by degree in descending order. This is because the depth of the scheduled circuit must be larger than the largest degree in the input graph and thus the more connected vertices have more influence on the depth of the circuit than a less connected vertex. Next, we will start the A star search with the root node having nothing mapped. Each subsequent node is generated and selected as follows: \\

\noindent 1. Select qubit q with the highest degree \\
2. For each unmapped location p, generate a child from the parent node in which qubit q is mapped on location p \\
3. Generate a cost for each of these nodes as follows:
\begin{enumerate}
  \item cost = max($cost_{\{q -> p\}}$, $cycle_{last}$)
  \item cost$_{\{q -> p\}} = max_{m \in mappedN(q)}(pattern(q,m))$
  \begin{itemize}
     \item $mappedN(q)$ is a list of mapped neighbours of q in input graph $G$
     \item pattern(q,m) is the cycle at which CPHASE(q,m) is scheduled in the pattern
     \item cost$_{\{q -> p\}}$ stands for the deepest cycle in which CPHASE(q,m) scheduled
     \item $cycle_{last}$ is the deepest scheduled cycle currently in the entire circuit
   \end{itemize}
\end{enumerate}
4. Select the node that minimizes cost and expand \\

Note that each node in the A Star tree is just a mapping between a qubit and a physical location. Thus, the height of the A Star tree would simply be N, the number of qubits in the graph. The heuristic function simply finds the latest time a qubit will execute with its neighbors given the current mapping in the pattern. If the latest cycle found is later than how long the circuit is currently scheduled to be, then that is set as the new cost (hence the max function). This allows our function to be admissible and move closer to an optimal solution with each node. 
%
\iffalse
\begin{algorithm}
\caption{A star based initial mapping}
\begin{algorithmic}[1] 
\STATE \textbf{Input: } Input graph G(V,E), V is a set of vertex and E is a set of edges
\STATE \textbf{Output: } Initial mapping $\pi$[]
\STATE Sort V by degree

\FOR{each v in V}
\STATE cost = INF
\FOR{$p \in unmap\_P()$}
    
    \STATE $cost_{v -> p} = max_{m \in mappedN(v)}(pattern(p,\pi[m]))$
    \IF{cost $\leq cost\_{p}$}
        \STATE $cost = cost_{p}$
        \STATE $\pi[v] = p$
    \ENDIF
\ENDFOR
\ENDFOR

\end{algorithmic}
\end{algorithm}
\fi
%

\noindent\textbf{The Subgraph Isomorphism Approach}

Subgraph isomorphism is another approach that can be used to find an initial mapping through the $CTAG$ pattern. In this approach, we represent both the input graph and the pattern as graphs. For the pattern, each edge(a,b) represents a CPHASE gate between $Q_x$-$Q_y$ where $Q_x$ is mapped to physical location a and $Q_y$ is mapped to physical location b. Figure \ref{fig:subgraphISO}(c) demonstrates the graph representation of Figure \ref{fig:subgraphISO}(a) which has the first 6 cycles of the $CTAG$ pattern of a clique-6 graph mapped on LNN. In this example, the edge between $Q_0$ and $Q_2$ in Figure \ref{fig:subgraphISO}(e) represents a CPHASE gate, $Q_0$-$Q_2$, that would be executed in cycle 4 of Figure \ref{fig:subgraphISO}(a). Notice that we can slowly build a graph, $G_{s}(i)$, from the cycles of the pattern where i denotes the cycle of the graph. For example, $G_{s}(1)$ would be a line graph like Figure \ref{fig:subgraphISO}(b) while $G_{s}(2N-2)$ would be a clique graph. 

The idea of subgraph isomorphism is to find a subgraph of $G_{s}(i)$ that is isomorphic to the input graph G. If they are isomorphic, then we can schedule graph G within i cycles. For example, if wanted to schedule the graph in Figure \ref{fig:subgraphISO}(d), we would see if it is isomorphic to Figure \ref{fig:subgraphISO}(b) which is the graph of the pattern after cycle 1. Since it is not isomorphic, we check again for cycle 5, in which we generate the graph in Figure \ref{fig:subgraphISO}(c). In this case, we are able to find a subgraph that is isomorphic to Figure \ref{fig:subgraphISO}(d). The corresponding subgraph is Figure \ref{fig:subgraphISO}(e) where we map edges 2-0-4-1-5-3 to A-B-C-D-E-F of Figure \ref{fig:subgraphISO}(d) and then edges 0-1 and 4-5 to match B-D and C-E. Thus, we can see that Figure \ref{fig:subgraphISO}(d) can be scheduled in 6 cycles.


\iffalse
\begin{algorithm}
\caption{Subgraph Isomorphsim based initial mapping}
\begin{algorithmic}[1] 

\STATE \textbf{Input: } Input graph G(V,E), V is a set of vertex and E is a set of edges
\STATE \textbf{Output: } Initial mapping $\pi$[]
\STATE pattern = $generate\_pattern(|V|)$;
\FOR{$i \in [0,|N|-1]$}
    \STATE graph G2 = construct\_G(pattern, i)
    \STATE // G2 is a graph from the first i CPHASE layers in the pattern
    \IF{is\_Isomor(G,G2)}
    \STATE return mapping
    \ENDIF
\ENDFOR

\end{algorithmic}
\end{algorithm}
\fi

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/subgraphISO.pdf}
    \caption{Subgraph isomorphic initial mapping: (a)The first six cycles of CTAG pattern of Clique6. (b) Graph constructed from edges at cycle 0 and 1 in the pattern.(c) Graph constructed from cycle edges at cycle 0,1,4, and 5. (d) Input problem graph with 6 vertices. (d) Subgraph of Fig.(c) which is isomorphic to Fig.(d). The letter near to the qubit represents mapping.}
    \label{fig:subgraphISO}
\end{figure}


\subsubsection{CTAG-H for General Graphs and Architecture}

\paragraph{Initial Mapping}
The initial mapping is important as the example shows in the last section. We will use the methods mentioned above to determine a good initial mapping in a linear path. Then we will follow the Hilbert curve to find such line embedding in the given architecture. Then, mapping the qubit will follow the order decided by CTAG-I. 

\paragraph{Step by Step Remapping}

Although our $CTAG$ pattern can effectively minimize the depth of a clique graph on an LNN architecture, it does so without any understanding of the architecture’s connectivity that is necessary for scheduling on more general architecture. We propose a second algorithm for more general input graphs that uses a more \textbf{H}euristic solution for the $CTAG$ pattern called $CTAG-H$. 

In Algorithm \ref{alg:CTAGH} line 1-2, $CTAG-H$ will take the graph G\_I(V1,E1) and architecture G\_A(V2,E2) as the input to return a scheduled circuit. In line 3, getInitialMapping() will generate a good initial mapping for the graph G\_I in a corresponding LNN architecture. Since we already have a good initial mapping, line 6, p=findPath() will find a line embedding in the architecture, so we can start scheduling the circuit by following the pattern. However, due to the drawback of simply using the pattern mentioned in section \ref{Pattern adaptation}, we will call function Partial\_pattern\_scheduling(p) in line 7 to start and pause the scheduling at a proper cycle, then start the heuristic process. The first step of the heuristic process begins in line 10. $Re$ is a set of executable CPHASE gates based on the current mapping. In line 11, We want to schedule as many gates as possible in one cycle, so we use the maximal matching in set Re to find maximum number of parallel gates and schedule those gates. In line 13, URe is a set of unscheduled gates, so we need to add swap gates to make those gates executable. The CHPASE gate that has shorter distance between two involved physical qubit has a higher scheduling priority. As a result, in line 14, we will sort gates in $URe$ by distance in ascending order and find a swap strategy for the gate in this order. There are two criteria to decide if the swap strategy is feasible. One is that the selected swap strategy cannot affect the current executable gate. The other one is that the selected swap strategy cannot affect any scheduled gates in that cycle. Then we will give all the feasible swap strategies a score. Each swap strategy ss of gate($n_{i}$,$n_{j}$) will update the qubit mapping of $n_{i}$ and $n_{j}$ from $p_{ni}$ and $p_{nj}$ to new physical qubits $p_{ni}^{'}$ and $p_{nj}^{'}$.  In line 17, for each swap strategy ss of gate($n_{i}$,$n_{j}$), 

$score =  \sum_{p_{nu}} dist(p_{ni}^{'},p_{nu}) +\sum_{p_{nu} } dist(p_{nj}^{'},p_{nu})$, 

where $p_{nu}$ is the physical qubit mapped by logical qubit $n_{u}$ and $n_{u}$ is the neighbor of $n_{i}$ and the corresponding CHPASE($n_{u}$, $n_{i}$) is not scheduled. Lastly, we will schedule one swap strategy $ss_{min}$ with minimal score for the corresponding CHPASE gate. 
 


\begin{algorithm}
\caption{$CTAG-H$: Pattern adapting heuristic scheduling }
\label{alg:CTAGH}
\begin{algorithmic}[1] 

\STATE \textbf{Input: } Input graph $G\_I(V1,E1)$; Architecture $G\_A(V2,E2)$
\STATE \textbf{Output: } Scheduled circuit

\STATE $\pi[]$ = getInitialMapping($G\_I$)
\STATE $edges = \{e| e \in E1 \}$
\WHILE{!edges.empty()}
\IF{p = findPath(G\_A)}
\STATE $e = Partial\_pattern\_scheduling(p)$
\STATE edges.remove(e)
\ENDIF
\STATE Re = $\{e(n1,n2)|(\pi[n1],\pi[n2]) \in E2 \}$
\STATE scheduleE = $\{e | e \in max\_matching(Re)\}$ 
\STATE schedule(scheduleE); edges.remove(scheduleE)
\STATE URe = E - Re
\STATE Sort(URe)
\FOR{edge(n1,n2) $\in$ URe}
    \FOR{ ss $\in$ swap\_strategies}
    \STATE score = get\_score(ss)
    \ENDFOR
    \STATE schedule $ss_{min}$
\ENDFOR

\ENDWHILE

\end{algorithmic}
\end{algorithm}

==> optimalMapper.tex <==
\section{Optimal QAOA Mapping Framework}
First of all, we want to do more investigation on finding the optimal solution for the QAOA compilation and later we propose a practical method for finding a near optimal solution. We adapt the A star framework since once a proper cost function is decided, the A star search can guarantee the optimal solution. 


\subsection{Detailed Explanation of the Pattern and Why It is guaranteed to cover all the edges}

\fixit{formal representation with figures and pseudo-code}

\fixit{intuitive explanation why it works}

\fixit{proof can be }

\subsubsection{Bounds} 
\subsubsection{Discussion of Pros and Conds}


\subsection{Adapting the Pattern}
\subsubsection{Factors to Consider}
\fixit{example to show that direct exact application may not be good enough and then talk about different factors}

\fixit{also talk about line embedding issue}

\subsubsection{General Methodology}

\section{Implementation details}
The A star search algorithm will traverse a true structure search space and schedule all the CPHASE gates and necessary SWAP gates to make the depth of scheduled circuit minimum. The search space is growing from a root node when the search is in process. We define cycle as a unit of time and one depth of scheduled circuit takes one cycle to execute.\\

Each node in the tree search space represents a circuit status including the current logical qubit to physical qubit mapping, part of circuit is already scheduled and the rest of gates that are still waiting to be scheduled. Each node has a cost assigned by the cost function which is used to evaluate the goodness of expanding that node. The node with the smallest cost will be expanded. Each edge between two nodes represents the circuit status transition, it stands for a possible combination of executable gates that are scheduled including CHPASE gates or SWAP gates. \\
The searching process starts at a root node which has nothing scheduled yet and it will be terminated when the search reaches a node where all the gates in the circuit are scheduled and other non-expanded nodes all have larger cost than the terminating node. Starting from the root node, the search space will be expanded by picking a node with minimum cost and  considering all the possible combinations of current executable gates including SWAP gates from that node. Each combination represents one node to node transition. If the node to node transition includes the SWAP gates, the mapping needs to be updated at the end of the transition. \\
The A star guided search algorithm works with a cost function as the guide. The cost function will evaluate each new node based on the circuit status at that node and give a cost. The cost function f(v) takes a node as input and consists of two parts g(v) and h(v) such that f(v) = g(v) + h(v). g(v) represents the length of path from the root to the node v which is the depth of the scheduled part of the circuit. h(v) is the heuristic cost as the lower bound of cost for scheduling the rest of the circuit, in order to guarantee the optimality.\\
Due to the commutativity feature of QAOA circuit, there is no such gate dependency as regular circuit. So the heuristic cost function has to be aware of this. We design a degree based heuristic cost function. No matter how the gate is scheduled, the degree of each qubit on that gate remains constant, useless SWAP gates are inserted. So we use the largest qubit’s degree as the lower bound of the scheduled circuit depth. However, we also need to consider the degree increased by the SWAP gates. So we estimate each unscheduled gate CPHASE(q1,q2) by checking the shortest distance between two corresponding qubits on the hardware. If the distance is I, this means at least I-1 swaps are needed for solving the hardware coupling constraint for that gate. By enumerating these pairs $(d1,d2) = \{(0, l-1), (1, l-2), (2, l-3), ….. \}$, each pair of (d1,d2) stands for one possible swap strategy, q1 will move d1 steps to q2 and q2 will move d2 steps to q1.  The degree of q1, d(q1) will be increased by d1 and the degree of q2,d(q2) will be increased by d2. The larger degree determines the minimum depth of circuit. For one swap strategy, the heuristic cost = max(d(q1)+d1, d(q2)+q2). We are trying to find the best swap strategy to minimize the circuit depth, so for all the swap strategies of one gate, we need min(max(d(q1)+d1, d(q2)+q2)) as the heuristic value of one gate. In order to make the heuristic value more close to the real optimal, the heuristic value of each gate will be compared to each other and find the largest one as the heuristic value of the unscheduled circuit which is max(min(max(d(q1)+d1, d(q2)+q2))). \\
Using this A star framework, we are able to find the optimal scheduling for any QAOA circuit. Even this method is not scale well for the large circuit, but it can find optimal scheduling for small benchmarks and help us conclude the pattern of Clique graphs in LNN architecture.
{\subsection{Bound and Scalability analysis}}
Analysis on directly applying the pattern: {\color{red}Compare with clique architecture.  In LNN, in 2XN in other architectures. Also considering graph type. }
Bounding analysis: Our pattern limits the depth of the scheduled circuit from $O(n^{2})$ to O(2n) where n is the number of qubits. When we schedule a QAOA circuit, we are not able to figure out how the optimal scheduling should be, especially when the benchmark is large.  but Not sure if the summarized pattern is optimal for a large number of qubits. But I claim that the summarized pattern is at most 2X worse than the optimal solution. We do not know how the real optimal is in LNN architecture, but we can know how the optimal is Because it keeps at least half of the cycles busy with the actual computation gates.
Our practical method in sparse graph scheduling can even give a better result. 
 {\color{red}Compilation time Worst case: brute force, current best, A star. In addition, those method does not guarantee the bound. Also compare on different architectures. Also consider difference graph types. } 
Our pattern guarantees the scalability of QAOA circuit scheduling. Currently, there is no way to find optimal scheduling in a reasonable time when the benchmark size is large in any physical architecture. Even though the A star search algorithm can accelerate the optimal solution searching process, the overhead of scheduling a large QAOA circuit is still unacceptable. However, if we can relax the constraint of looking for a scheduling with at worst 2N depth, the overhead of such scheduling is constant. By applying our pattern  LNN or 2D
Through the correctness proof, we can say that  
The pattern guarantees that as long as we can find a path with enough qubit in the architecture, we can schedule the circuit with constant time and at most 2N depth.


\subsection{Patterns for Clique graph}
When using QAOA to solve MAX-CUT problems, one specific type of graph is non-neglectable, clique graph. Because all the graphs are subgraphs of clique graphs, if we can come up with a good mapping for a clique graph, we can easily compile its subgraph by removing some corresponding CPHASE gates and SWAP gates. By using our QAOA optimal compiler, we surprisingly found that there are specific patterns when we compile the QAOA circuit of clique graphs on Linear Nearest Neighbour(LNN) architectures. \\
{\textbf{Pattern on LNN: }}starting with the initial mapping, logical qubit $q_i$ mapped to physical qubit $Q_i$. The movement of each logical qubit in a 3-1-3 pattern. For the first 3 cycles, $q_i$ does not move. At the forth cycle, $q_i$ moves to one of its nearest neighbours. At the next 3 cycles, $q_i$ moves to one of its nearest neighbours again. Each three cycles, qi is mapped to the same Qj , then qi starts moving. If the i is an even number, it will move upward until it reaches the boundary then start moving downward. If the i is an odd number, it will move downward until it reaches the boundary then start moving upward. After the first three cycles, qi moves one step. If qi is already in the boundary, then qi does not move at the forth cycle. In the next three cycles, qi will turn the direction and move to the nearest neighbour. The first and the second cycles in this 3-1-3 pattern only contain CPHASE gates. At the first cycle, a sequence of CPHASE is starting at the first logical qubit from top to bottom until no more gates can be applied. At the second cycle, a sequence of CPHASE is starting at the second logical qubit from top to bottom until no more gates can be applied. At the third cycle, a sequence of SWAP gates are applied at the same pair of qubits as the second cycle. The next three cycles repeat the same pattern. For the cycle in the middle, a sequence of SWAP gates are applied to the same pair of qubits as the forth cycle.
\begin{algorithm}
\caption{Pattern for Clique n on LNN}
\begin{algorithmic} 
\STATE n: number of vertex in Clique graph
\STATE $\pi[] = [0, 1, ..., n-1]$
\STATE 
\FOR{t = 0; t $<$ 2n-2; t $++$}
\IF{t mod 4 == 0}
\FOR{p = 0; p $<$ n; p = p + 2}
\STATE  $CPHASE(\pi[p], \pi[p+1])$
\ENDFOR 
\ELSIF{t mod 4 == 1}
\FOR{p = 1; p $<$ n; p = p + 2}
\STATE  $CPHASE(\pi[p], \pi[p+1])$
\ENDFOR
\ELSIF{t mod 4 == 2}
\FOR{p = 1; p $<$ n; p = p + 2}
\STATE  $SWAP(\pi[p], \pi[p+1])$
\STATE  $SWITCH(\pi[p], \pi[p+1])$
\ENDFOR
\ELSIF{t mod 4 == 3}
\FOR{p = 0; p $<$ n; p = p + 2}
\STATE  $SWAP(\pi[p], \pi[p+1])$
\STATE  $SWITCH(\pi[p], \pi[p+1])$
\ENDFOR
\ENDIF
\ENDFOR

\end{algorithmic}
\end{algorithm}


\subsection{Search Space}

